Adaptive Methods for Real-World Domain Generalization

Invariant approaches have been remarkably successful in tackling the problem of domain generalization, where the objective is to perform inference on data distributions different from those used in training. In our work, we investigate whether it is possible to leverage domain information from the unseen test samples themselves. We propose a domain-adaptive approach consisting of two steps: a) we first learn a discriminative domain embedding from unsupervised training examples, and b) use this domain embedding as supplementary information to build a domain-adaptive model, that takes both the input as well as its domain into account while making predictions. For unseen domains, our method simply uses few unlabelled test examples to construct the domain embedding. This enables adaptive classification on any unseen domain. Our approach achieves state-of-the-art performance on various domain generalization benchmarks. In addition, we introduce the first real-world, large-scale domain generalization benchmark, Geo-YFCC, containing 1.1M samples over 40 training, 7 validation, and 15 test domains, orders of magnitude larger than prior work. We show that the existing approaches either do not scale to this dataset or underperform compared to the simple baseline of training a model on the union of data from all training domains. In contrast, our approach achieves a significant improvement.

==> sec_approach_final.tex <==
% \begin{figure*}[htb]
% \centering
% \includegraphics[width=\linewidth]{main.pdf}
% \caption{A visual representation of our two-step training pipeline. Figure A describes the prototypical training process (Step 1), which is followed by training the \textit{adaptive} classifier (Figure B).}
% \label{fig:myfigure}
% \end{figure*}

We assume that each \textit{domain} $D \in \cD$ is a probability distribution over $\cX \times \cY$, i.e., the product of the input space $\cX$ and output space $\cY$, and there exists a \textit{mother} distribution $\fP$ which is a measure over the space of domains $\cD$. A \textit{training domain} $\widehat D(n)$ is obtained by first sampling a domain $D$ from $\fP$, and then sampling $n$ points ($X$ and $Y$) from $\cX \times \cY$ following $D$. A training set can then be constructed by taking the union of $N$ such domains $(\widehat{D}_i(n))_{i=1}^N$. Correspondingly, any test domain $\widehat D_T(n_T)$ is also constructed by first drawing a sample $D_T \sim \cD$ and then drawing $n_T$ samples from $D_T$, and discarding the labels.

% The problem of domain generalization can then be formally defined as: 

% {\textit{Definition: Given $N$ training domains $(\widehat{D}_i(n))_{i=1}^N$ sampled from $\fP$, train a model that performs well on any unseen domain $\widehat D_T(n_T)$ also sampled from $\fP$.}}
% ABHI COMMENT: NOt sure if we can say that definition since we also want to minimize expected risk over all domains.

\begin{algorithm*}[t!]
\footnotesize
\caption{Adaptive Training Pseudocode}
\begin{minipage}{.5\linewidth}
\begin{flushleft}
\label{alg:proto_algo}
\textsc{Prototype Training:}\\
\textbf{Input:} $N$ domains $(D_i)_{i=1}^N$ with $n$ samples each. $N_t$ : domains sampled each batch, $N_s$: support examples to compute embedding, $N_q$: query examples per batch.
\textbf{Output}: Embedding neural network $\Phi_\cD : \cX \rightarrow \bbR^{d_D}$.\\
\begin{algorithmic}%[1] enables line numbers
\STATE \textbf{Initialize}:  weights $\btheta$ of $\Phi_\cD$ randomly.
\FOR{Round $t = 1$ to $T$}
\STATE $D_t \leftarrow \textsc{Randomly Sample}(N, N_t)$.  // sample $N_t$ domains
\FOR{Domain $d$ in $D_t$}
\STATE $\cS_d \leftarrow \textsc{Randomly Sample}(D_d, N_s)$. // sample support points
\STATE $\cS_q \leftarrow \textsc{Randomly Sample}(D_d, N_q)$. // sample query points
\STATE $\widehat\bmu_d \leftarrow \frac{1}{N_s}\sum_{\x \in \cS_d} \Phi_\cD(\x; \btheta)$. // compute prototype
\ENDFOR
\STATE $J_\btheta(t) \leftarrow 0$.
\FOR{Domain $d$ in $D_t$}
\FOR{$\x \in \cS_q$}
\STATE // update loss
\STATE $J_\btheta(t, \x) \leftarrow d(\Phi_\cD(\x), \widehat\bmu_d)$. 
\STATE $J_\btheta(t, \x) \leftarrow J_\btheta(t, \x) + \log\underset{d' \in D_t}{\sum}\exp\left(-d(\Phi_\cD(\x), \widehat\bmu_{d'})\right)$.
\STATE $J_\btheta(t) \leftarrow J_\btheta(t) + \frac{1}{N_sN_q}J_\btheta(t, \x)$.
\ENDFOR
\ENDFOR
\STATE $\btheta \leftarrow \btheta + \alpha\nabla(J_\btheta(t))$. // gradient descent step
\ENDFOR
\RETURN $\btheta$.
\end{algorithmic}
\textsc{Prototype Computation $(D, \Phi_\cD, N_p)$:}\\
\textbf{Input}: Trained prototype network $\Phi_\cD$ with weights $\btheta^*$, Domain $D$. Number of points $N_p$ to create prototype.\\ \textbf{Output}: Prototype $\bmu(\widehat D)$.
\begin{algorithmic}%[1] enables line numbers
\STATE $\cS_p \leftarrow$ \textsc{RandSample}$(N_p, D_d)$. // sample points
\RETURN $\bmu(\widehat D_d) \leftarrow \frac{1}{N_p}\sum_{\x \in D_d} \Phi_\cD(\x, \btheta^*)$.
\end{algorithmic}
\end{flushleft}
\end{minipage}
\hspace{5pt}
\begin{minipage}{.52\linewidth}
\begin{flushleft}
\textsc{Adaptive (Main) Training:}\\
\textbf{Input}: Trained prototype network $\Phi_\cD$ with weights $\btheta^*$, Domains $(D_i)_{i=1}^N$. \textbf{Output}: Feat. extractor $F_{\text{ft}}$ with weights $\bomega_{\text{ft}}$, classifier $F_{\text{mlp}}$ with weights $\bomega_{\text{mlp}}$.
\begin{algorithmic}
\STATE // compute prototypes for training domains
\FOR{Domain $d$ from $1$ to $N$}
\STATE $\bmu(\widehat D_d) \leftarrow$ \textsc{Prototype Computation}$(D_i, \Phi_\cD, N_p)$.
\ENDFOR
\STATE Create augmented dataset $(\widetilde D_i)_{i=1}^n$ (Equation~\ref{eqn:augmented_dataset}).
\FOR{SGD round $t=1$ to $T$}
\STATE Sample batch $(\x, \bmu, y)$ from augmented dataset.
\STATE $\Phi_\cX(\x) \leftarrow F_{\text{ft}}(\x; \bomega_{\text{ft}})$. // compute image features
\STATE $\Phi(\x, \bmu) \leftarrow \textsc{Concat}(\Phi_\cX(\x), \bmu)$. // concatentate features
\STATE $\hat y \leftarrow F_{\text{mlp}}(\Phi(\x, \bmu); \bomega_{\text{mlp}})$. // compute predictions
\STATE $J_{\bomega}(t) \leftarrow \textsc{CrossEntropy}(\hat y, y)$. // compute loss
\STATE // gradient descent steps
\STATE $\bomega_{\text{ft}} \leftarrow \bomega_{\text{ft}} + \alpha \nabla_{\bomega_{\text{ft}}} J_{\bomega}(t)$.
\STATE $\bomega_{\text{mlp}} \leftarrow \bomega_{\text{mlp}} + \alpha \nabla_{\bomega_{\text{mlp}}} J_{\bomega}(t)$.
\ENDFOR
\RETURN $\bomega^* \leftarrow (\bomega_{\text{ft}}, \bomega_{\text{mlp}})$.
\end{algorithmic}
\textsc{Adaptive Inference:}\\
\textbf{Input}: Trained networks $\Phi_\cD, F_{\text{ft}}, F_{\text{mlp}}$ with weights $\btheta^*, \bomega^*_{\text{ft}}, \bomega^*_{\text{mlp}}$.\\ 
Set of $N$ points $D$ from the same domain.\\
\textbf{Output}: Predictions $y$.
\begin{algorithmic}
\STATE // first compute prototype
\STATE $\bmu(\widehat D) \leftarrow$ \textsc{Prototype Computation}$(D, \Phi_\cD, N)$.
\STATE $\Phi_\cX(\x) \leftarrow F_{\text{ft}}(\x; \bomega_{\text{ft}})$. // compute image features
\STATE $\Phi(\x, \bmu) \leftarrow \textsc{Concat}(\Phi_\cX(\x), \bmu(\widehat D))$. // concatentate features
\STATE $\hat y \leftarrow F_{\text{mlp}}(\Phi(\x, \bmu); \bomega_{\text{mlp}})$. // compute predictions
\RETURN $\hat y$.
\end{algorithmic}
\end{flushleft}
\end{minipage}
\end{algorithm*}
Our approach involves learning an \textit{adaptive} classifier, i.e., a function $F: \mathcal X \times \mathcal D \rightarrow \mathcal Y$ that takes \textit{both} the point $\x$ and the domain $D$ of $\x$ into consideration. Our goal is to make sure that for any test domain $D_T$, the resulting classifier $f_T = F(\cdot, D_T)$ from $F$ lies close to $\hat f_T$. We assume that a small set of unsupervised data is available from $D_T$ to characterize $F(\cdot, D_T)$ from $F$\footnote{This assumption is trivially satisfied by the test set itself. In practice, we can also collect a small separate set of points easily during deployment.}. Note that during training, we do not have access to $D_T$ and hence we do not perform any \textit{transductive learning}, unlike unsupervised domain adaptation.
The main challenge in creating such a function $F$ is that it is non-trivial to learn a function that operates on the space of arbitrary probability distributions. To alleviate this issue, we follow a two step approach:

\noindent{(A) \textbf{Computing domain embeddings:}} We first learn a \textit{domain embedding} function  $\Phi_\cD : D \rightarrow \bbR^{d_\cD}$, that maps any domain $D \in \cD$ to a finite vector. Ideally, we want this embedding to be learned from a few samples belonging to the domain (i.e., \textit{low-shot}), and hence we leverage the popular technique of \textit{prototypical learning}~\cite{snell2017prototypical}. We further demonstrate in Section~\ref{sec:theory} the advantages of the domain embedding approach via the theory of kernel mean embeddings~\cite{muandet2016kernel}, a formalization that can represent probablility distributions as vectors in a suitable Hilbert space.

% We utilize kernel mean embeddings (KME)~\cite{muandet2016kernel}, a mathematical formalization that enables the representation probability distribution as the average of feature vectors in a Hilbert space computed from samples drawn from the probability distribution itself. The objective is to learn a function $\Phi$ (i.e., domain embedding), that maps any domain $D \in \cD$ (including empirical domains) to a finite vector, i.e., $\Phi : D \rightarrow \bbR^{d_\cD}$.

\noindent{(B) \textbf{ERM using augmented inputs:}} Once we have a suitable domain embedding $\Phi$, we learn a neural network $F$ directly over the \textit{augmented input} $(\x, \Phi(\widehat D))$, where $\x$ is a point from the domain $\widehat D$, using regular ERM (Equation~\ref{eq:erm}). 

\noindent \textbf{Inference:} Inference on an unseen domain $\widehat D_T$ is done by using unsupervised samples (or the test set when none are present) from $\widehat D_T$ and the learned function $\Phi$ from (A) to compute the domain embedding $\Phi(\widehat D_T)$. We then provide the computed embedding as an additional input to the model $F$ from (B) to get the \textit{adaptive} model $F(\cdot, \Phi(\widehat D_T))$.

%Our prototypical training proceeds by randomly sampling a batch of points from each domain, and running the feedforward operation $\Phi_\cD$ on them. In practice, $\Phi_\cD$ is a neural network. Then, a subset of points from each domain are used to create an approximation $\bmu(\widehat D)$ for each domain $D$, and the remaining points are used for $N$-way classification.
% The features extracted from the second set of points are used to classify them into their respective domains. We produce a distribution over the $N_t$ domains for any input point $\x$ in this second set, based on a softmax distance to the approximate embedding for each domain:
\subsection{Prototypical Domain Embedding}
\label{sec:prototype}
Our domain embedding $\Phi_\cD$ is trained with stochastic gradient descent (SGD) using the technique of \textit{prototypical learning}. At each iteration, we first sample a subset of $N_t$ domains from the training domains. Next, we sample two sets of points from each domain. The first set is used to obtain the embedding for the domain, by feedforward through the network $\Phi_\cD$ and averaging (Eq.~\ref{eq:emb}). This results in an approximate embedding $\bmu(\widehat D)$ for each domain $D$ sampled during this iteration. Every point $\x$ in the second set is assigned a probability of beloging to a domain $D$ as follows. 
\begin{align}
    p_\btheta(\x \in D) = \frac{\exp\left(-\lVert \bmu(\widehat D) - \Phi_\cD(\x)\rVert_2^2 \right)}{\sum_{i=1}^{N_t} \exp\left(-\lVert \bmu(\widehat{D}_i) - \Phi_\cD(\x)\rVert_2^2\right)}.
\end{align}
Learning proceeds by minimizing the negative log-likelihood $J(\btheta) = -\log p_\btheta(\x \in D_\x)$ for the correct domain $D_\x$ from which $\x$ was sampled. After training, we obtain the final model parameters $\btheta^*$. For each domain $\widehat{D}_i(n)$, the \textit{domain prototype} (embedding) is constructed as:
\begin{equation}
    \bmu(\widehat{D}_i(n)) := \frac{1}{n}\sum_{j=1}^{n} \Phi_\cD(\x; \btheta^*). \label{eqn:final_prototype}
\end{equation}
Prototype training and construction is completely unsupervised, as we do not utilize any class labels as long as we are provided the inputs partitioned by domains. We repeat \textit{only} Equation~\ref{eqn:final_prototype} for each test domains as well (no retraining).

\subsection{ERM on Augmented Inputs}
\label{sec:augtrain}
Once we have the domain prototype for each training domain from the previous step, we create the \textit{augmented} training set by appending the corresponding prototype to each input. We obtain the training set $\widetilde\cS_\trn = \cup_{i=1}^{N} \widetilde{D}_i$, where, 
\begin{equation}
\widetilde{D}_i = \left(\x_{ij}, \bmu(\widehat{D}_i), y_{ij}\right)_{j=1}^{n}.
\label{eqn:augmented_dataset}
0\end{equation}

The second step is to then train the \textit{domain-adaptive} classifier $F$ over $\widetilde\cS_\trn$ using regular ERM training. $F$ consists of two neural networks (Figure~\ref{fig:myfigure}). The first network $F_{\text{ft}}$  with weights $\bomega_{\text{ft}}$ takes $\x$ (image) as input and outputs a feature vector $\Phi_\cX(\x)$. We then concatenate the image feature $\Phi_\cX$ with the domain embedding $\bmu(D)$ and pass through the second network $F_{\text{mlp}}$ which predicts the class label $y$. We refer to this approach as \daerm. In Section~\ref{sec:smallscale}, we present a few variants that combine the complimentary nature of adaptive and invariant approaches.
 
When testing, we first compute the domain prototypes for a test domain $\widehat D_T$ (Equation~\ref{eqn:final_prototype}) using a small number of unlabeled examples\footnote{We can also use a small sample of the total test set to create $\bmu(\widehat D_T)$.}, and then produce predictions via $F(\cdot, \widehat D_T)$. Alternatively, it is possible to decouple the prototype construction and inference procedures in the test phase (since we can use unsupervised samples obtained \textit{a priori} to construct prototypes). Note that once the prototype $\bmu(\widehat D_T)$ is computed, we only need the adapted classifier $F (\cdot, \widehat D_T)$ for inference, not the prototypical network.
\subsection{Theoretical Guarantees}
\label{sec:theory}
Here we provide an abridged summary of our theoretical contributions, and defer the complete results and proofs to the appendix. We first provide some intuition for our approach. Consider a family of functions $\cF$. For each $D \in \cD$, the optimal classifier $f_D$ in $\cF$ (for some loss function $\ell$) can be given by $ f_D = \argmin_{f \in \cF} \bbE_{(\x, y) \sim D}[\ell(f(\x), y)]$. We denote the optimal empirical risk minimization (ERM) classifier for each domain $\widehat D_i$ in the training set domain $\widehat D_i(n)$ as $\hat f_i = \argmin_{f \in \cF} \bbE_{(\x, y) \sim \widehat D(n)}[\ell(f(\x), y)]$ . The \textit{universal} expected risk minimizer (i.e., classifier minimizing overall risk over $D \sim \fP$) can then be given by $f_*$ such that,
\begin{equation}
f_* = \argmin_{f \in \cF} \bbE_{D \sim \fP}\bbE_{\x, y \sim D}[\ell(f(\x), y)].
\label{eq:erm}
\end{equation}
Typically, the optimal classifier for $D_T$ within $\cF$ may be far from the (non-adaptive) universal classifier $\hat f_*$, a distance which we call the ``adaptivity gap''. A visual heuristic representation of the above intuition is provided in Figure~\ref{fig:intuition}. Ideally, we would like the classifier to be chosen closer to $\hat f_T$ such that it obtains lower error. Note that the \textit{adaptivity gap} may be large even when the training set contains samples close to $\hat f_T$ (in the figure, this refers to functions $\hat f_7$ and $\hat f_8$), since the \textit{universal} classifier minimizes overall risk.

We employ an \textit{adaptive} approach to learn a function $F: \cD \times \cX \rightarrow \bbR$. To understand how such a function can be learnt, we leverage  the nonparametric method of \textit{kernel mean embeddings} (KME)~\cite{muandet2016kernel}, an elegant approach to embed distributions into vector spaces. Let $D_X$ denote the marginal of $\cX$ under $D$, i.e., only the distribution of points $\cX$ in $D$. The fundamental idea behind KMEs is to consider each probability distribution $D_X \in \cD_\cX$ as a member of a reproducing kernel Hilbert space (RKHS) $\cH(\cX)$ with some kernel $k$ and feature $\Phi_\cD : \bbR^d \rightarrow \bbR^{d_D}$. Then, the KME of any distribution $D \in \cD$ with marginal $D_X$ can be given as,
\begin{equation}
    \bmu(D_X) = \int_{\cX} \Phi_\cD(\x)dD_X(\x).
\end{equation}
The strength of this approach is that, if a suitable $\Phi_\cD$ is chosen (see below), then it is possible to learn a function over the space of distributions $\cD$ via the average feature embedding of samples drawn from $D$. Hence, we propose to learn both a domain embedding $\bmu$ using features $\Phi_\cD$ and the target function $F(\cdot, \bmu(\cdot))$, such that when any domain $D$ is presented, we can provide an \textit{adapted} function $F(\cdot, {\bmu}(D))$.

We learn a neural network $\Phi_\cD :\cX \rightarrow \bbR^{d_D}$, parameterized by weights $\btheta$, and then compute the $n$-sample \textit{empirical} KME $\bmu$ of each training domain $\widehat D$ as:
% \in \cS_\trn$ as:
\begin{equation}
    \bmu(\widehat D) = \frac{1}{n}\sum_{\x \in \widehat D} \Phi_\cD(\x ; \btheta).
\label{eq:emb}
\end{equation}
\textbf{Low-Shot Domain Prototypes}.
To be useful in classification, we require $\bmu$ to satisfy two central criteria:\vspace*{0.05in}\\
\noindent (A) \textbf{Expressivity}: $\bmu$, and consequently, $\Phi_\cD$, must be expressive, i.e., for two domains $D$ and $D'$, $\lVert \bmu(D) - \bmu(D') \rVert_2$ must be large if they are very distinct (i.e., domain shift), and small if they are similar. For example, if $\Phi_\cD$ is constant, the KME will provide no additional information about $D$, and we can expect the \textit{expected risk} itself to be large in this case, equivalent to non-adaptive classification. To make this argument rigorous, we present our first theoretical result, a generalization bound that controls the gap between the training error $\widehat L_{n, N}(F)$ and test error $L(F)$ (RHS of Eqn.~\ref{eq:erm}) for $F$ that is \textit{adaptive}, i.e., a function of $\cX \times \cD$ and lies in the Hilbert space determined by some kernel $\kappa$. We build on the framework of~\cite{blanchard2011generalizing} and extend their results to a more general class of kernel functions.
\begin{theorem}(error bound, informal) Let $F$ be an adaptive classifier defined over $\cX \times \cD$ that lies in an RKHS $\cH_\kappa$ such that $\lVert F \rVert_{\cH_\kappa} \leq 1$. Then, we have, with high probability that $|L(F) - \widehat L_{n, N}(F)| \lesssim \widetilde{\mathcal O}\left(((\log N) /n)^{1/2} + N^{-1/2}\right)$.
\label{thm:risk_bound}
\end{theorem}
Now, Theorem~\ref{thm:risk_bound} controls the difference between \textit{training error} $\widehat L_{n, N}(F)$ and test error $L(F)$ for a class of functions $\cF$ such that $\lVert f \rVert_{\cH_\kappa} \leq 1$. Informally, this suggests that if the feature $\Phi_\cD$ is not expressive, the class of functions $\cF$ itself is very small, and hence even the best achievable test error $L(F)$ will be large, regardless of training error $\widehat L_{n, N}(F)$.
\vspace*{0.05in}\\
\noindent (B) \textbf{Consistency}: Next, $\Phi$ must have little dependence on both the choice, and the number of samples $\x$ used to construct it. This is desirable as during both training and testing, we only have access to the empirical distribution $\widehat{D}$ corresponding to any domain $D$. This can be achieved, if we learn $\Phi_\cD$ such that for any sample $\x$ from domain $D$, $\Phi_\cD(\x)$ is strongly clustered around the KME $\bmu(D)$. Our second result makes this requirement rigorous, as a concentration bound on the $n$-point approximation error of $\bmu$.
\begin{theorem}($\bmu$ approximation, informal)
For any domain $D$ and feature $\Phi$  such that $\bbE_{\x \sim D}[\lVert\Phi(\x)\rVert_2^2] \leq \sigma^2$, let the corresponding empirical dataset be $\widehat D(n)$, let $\bmu(D)$ be the true mean embbeding and $\bmu(\widehat D)$ be its approximation. Then with high probability, $\lVert \bmu(D) - \bmu(\widehat D) \rVert_\infty \lesssim \widetilde{\mathcal O}(\sigma/\sqrt{n})$\footnote{The $\widetilde\cO$ notation hides polylogarithmic factors and failure probability.}. 
\label{thm:prototype}
\end{theorem}
For low error, therefore, the variance $\sigma$ must be small for each  $D \in \cD$, i.e., the embedding $\Phi_\cD$ must be consistent. These two exact constraints have been explored previously in the area of low-shot classification, by an algorithm known as \textit{prototypical learning}~\cite{snell2017prototypical}. Prototypical learning learns a set of \textit{prototypes} (ref. KMEs) for each class in low-shot classification, and predicts the label of a new point as the class label of its nearest prototype. We know that prototypical learning induces a soft clustering of points based on their categories (see Section 2.3 of Snell~\etal\cite{snell2017prototypical}), and ensures that the features learnt are centered around the prototypes (i.e., consistent), and the cluster centers (prototypes) are far apart (i.e., expressive). We therefore adopt a \textit{domain-level} prototypical learning model, where we essentially run the prototypical network algorithm (Algorithm 1 of~\cite{snell2017prototypical}) but using the domain identities as the labels.


==> sec_experiments.tex <==
We compare our algorithm with various recent algorithms on domain generalization problems both at the small-scale (i.e., fewer domains and classes per domain, and significant hyperparameter tuning is possible) and at the real-world (large-scale) level (i.e., many train and test domains, large class imbalance across domains, and extensive hyperparameter tuning is not possible). All benchmark algorithms are implemented from the \textsc{DomainBed}~\cite{gulrajani2020search} suite with the hyperparameter value ranges suggested therein.

\vig{Replace above para with: We compare our method with various recent algorithms for domain generalization, both at the small-scale and the real-world (large-scale) level. At a smaller scale with fewer domains and classes per domain, significant hyperparameter tuning is possible; unlike the real-world setup with many domains that have large class imbalance between them. All benchmark algorithms are implemented from the \textsc{DomainBed}~\cite{gulrajani2020search} suite with the hyperparameter value ranges suggested therein.}

We denote our implementation of domain-aware training as \textbf{DA-ERM}, i.e., \textit{domain-aware} empirical risk minimization (since we do not add additional penalties beyond regularized empirical risk in the training objective). Our algorithm is implemented as follows. Consider a domain generalization problem with $N_{\text{tr}}$ training domains and $N_{\text{te}}$ test domains, with the $i^{th}$ training (resp. test) domain having $n_{i}^{\text{tr}}$ (resp. $n_{i}^{\text{te}}$) examples. First, we train a prototypical classifier on the training data $((\x_{ij}, i)_{j=1}^{n_i^{\text{tr}}})_{i=1}^{N_{\text{tr}}}$ to predict the domain label from the input. This network is a ResNet-50~\cite{he2016deep} neural network pre-trained on ImageNet-12~\cite{deng2009imagenet}, truncated after the \texttt{pool5} layer, and an additional fully-connected layer (of variable dimension $d_{\text{feat}}$) appended to the output \vig{with a randomly initialized fully-connected layer (of variable dimension) appended to it}, followed by a ReLU~\cite{agarap2018deep} activation.

We then compute the \textit{domain prototype} for each of the $N_{\text{tr}}$ domains (Equation~\ref{eqn:final_prototype}) and create the augmented input (see Section~\ref{sec:training_inference}). The classifier operates on the augmented input as follows. We first have an image feature extractor (with network architecture identical to the prototype case), the output of which is concatenated to the domain prototype. This concatenated input is passed through a \textit{bottleneck} fully-connected layer (of dimensionality $d_{\text{bn}}$ and then a final classifier producing the logit values for all classes. Note that during training of the classifier, we allow fine-tuning of the image feature extractor, however, the prototypes themselves are fixed for all domains. \vig{Is this a repetition of the approach section? Is this paragraph needed?}

\begin{table*}[th!]
\centering
\rowcolors{3}{blue!10}{white}
\begin{tabular}{ccccccc}
\hline
\hline
\textbf{Algorithm} & VLCS        & PACS                 & Office-Home          & Domain-Net           & 
Terra Incognita        & Average               \\
\hline
ERM      &76.7 $\pm$ 0.9         &83.2 $\pm$ 0.7        &67.2$\pm$ 0.5         &41.1$\pm$ 0.8         &
46.2 $\pm$ 0.3         &62.9 $\pm$ 0.6         \\
IRM      &76.9 $\pm$ 0.5         &82.8 $\pm$ 0.5        &67.0$\pm$ 0.4         &35.7$\pm$ 1.9         & 
43.8 $\pm$ 1.0         &61.2 $\pm$ 0.8         \\
DRO      &77.3 $\pm$ 0.2         &83.3$\pm$ 0.3         &66.8$\pm$ 0.1         &33.0$\pm$ 0.5         &
42.0 $\pm$ 0.6         &60.4 $\pm$ 0.4         \\
Mixup    &78.2 $\pm$ 0.6         &83.9$\pm$ 0.8         &68.3$\pm$ 0.4         &40.2$\pm$ 0.4         &
46.2 $\pm$ 0.5         &63.3 $\pm$ 0.7         \\
MLDG     &76.8 $\pm$ 0.4         &82.6$\pm$ 0.6         &67.7$\pm$ 0.3         &42.2$\pm$ 0.6         & 
46.0 $\pm$ 0.4         &63.0 $\pm$ 0.4         \\
CORAL    &77.3 $\pm$ 0.3         &83.3$\pm$ 0.5         &68.6$\pm$ 0.1         &42.1$\pm$ 0.7         &
47.7 $\pm$ 0.3         &63.8 $\pm$ 0.3         \\
MMD      &76.1 $\pm$ 0.7         &83.1$\pm$ 0.7         &67.3$\pm$ 0.2         &38.7$\pm$ 0.5         &
45.8 $\pm$ 0.6         &62.2 $\pm$ 0.6         \\
C-DANN   &73.8 $\pm$ 1.1         &81.4$\pm$ 1.3         &64.2$\pm$ 0.5         &39.5$\pm$ 0.2         &
40.9 $\pm$ 0.7         &60.1 $\pm$ 0.9         \\ 
\hline
DA-ERM   &78.0 $\pm$ 0.2         &84.1$\pm$ 0.5         &67.9$\pm$ 0.4         &43.6$\pm$ 0.3         &
47.3 $\pm$ 0.5         &64.1 $\pm$ 0.8         \\
DA-MMD   &\textbf{78.6 $\pm$ 0.5}&84.4$\pm$ 0.3         &68.2$\pm$ 0.1         &43.3$\pm$ 0.5         &
47.9 $\pm$ 0.4         &64.5 $\pm$ 0.5         \\
DA-CORAL &78.5 $\pm$ 0.4         &\textbf{84.5$\pm$ 0.7}&\textbf{68.9$\pm$ 0.4}&\textbf{43.9$\pm$ 0.3}&
\textbf{48.1 $\pm$ 0.3}&\textbf{64.7 $\pm$ 0.6}\\ 
\hline
\hline
\end{tabular}
\caption{Comparative evaluations using the \textsc{DomainBed} domain generalization benchmark suite.}
\label{tab:exp_small_scale}
\end{table*}
\subsection{Small-Scale Benchmarks} We conduct small-scale benchmark comparisons carefully following the \textsc{DomainBed} suite for domain generalization~\cite{gulrajani2020search}, which contains 7 datasets in total. This paper focuses specifically on real-world domain generalization, and hence we select the 5 larger datasets (VLCS~\cite{fang2013unbiased}, PACS~\cite{li2017deeper}, Office-Home~\cite{venkateswara2017Deep}, Domain-Net~\cite{peng2019moment} and Terra Incognita~\cite{beery2018recognition}) for our experiments, and discard the synthetic MNIST-based~\cite{lecun1998mnist} datasets.

The training details and hyperparameter ranges for our algorithm as well as other benchmarks can be found in the Appendix. In the small-scale setting, we select hyperparameters by \textit{leave one domain out} cross validation, the de facto technique for model selection for domain generalization, wherein we run $N_{\text{tr}}$ trials of each hyperparameter setting, setting one domain for testing and the rest for training, and selecting the set of hyperparameters that maximize validation accuracy over the training domains, averaged over all $N_{\text{tr}}$ trials. Performance under alternative techniques for model selection are presented in the Appendix.

\textbf{Domain Mixup}. Since the small-scale datasets have typically 4 and at most 7 domains in total (1 of which is used as testing), the resulting training set (of domains) is not representative enough to learn a sufficiently discriminatory domain prototype. To alleviate this issue, we introduce \textit{mixup}~\cite{zhang2017mixup} in the prototype training step, where, for each batch of points from training domains, we construct \textit{synthetic} domains by averaging points belonging to different domains and providing that as additional samples (belonging to a new domain). For example during training, if we have a batch with $N$ points from $n$ training domains, we will sample $n$ synthetic domains by averaging pairs of points between random domains to create $2N$ total points from $2n$ domains. The blending ratio for each synthetic domain is randomly chosen uniformly between $(0.2, 0.8)$.

The results are summarized in Table~\ref{tab:exp_small_scale}, where each experiment is averaged over 8 independent trials (for our algorithm, this includes retraining of the domain prototypical network). We observe an average improvement of \textbf{1.87\%} in accuracy across all 5 datasets over existing methods, where the improvement is more substantial in Domain-Net~\cite{peng2019moment} and Terra Incognita~\cite{beery2018recognition} datasets, that have a larger number of domains. This can be attributed to the increased diversity in the training data, which allows us to construct a strong covering of the space of domains.
\begin{table*}[th!]
\rowcolors{3}{blue!8}{white}
\centering
\begin{tabular}{ccccccc}
\hline
\hline
\multirow{2}{*}{Algorithm} & \multicolumn{3}{c}{DG - ImageNet $(K=100, N_\trn=50)$} & \multicolumn{3}{c}{Geo - YFCC (Top-$5$)} \\
         & Train                 & Val                   &  Test                 & Train                  & Val                    & Test                   \\
         \hline
ERM      &90.1 $\pm$ 1.6         &77.2 $\pm$ 1.7         &76.9 $\pm$ 0.4         &\textbf{56.3 $\pm$ X.XX}&46.2 $\pm$ X.XX         &48.2 $\pm$ X.XX         \\
Mixup    &89.5 $\pm$ 1.8         &77.9 $\pm$ 1.9         &78.2 $\pm$ 0.8         &X.XX $\pm$ X.XX         &X.XX $\pm$ X.XX         &X.XX $\pm$ X.XX         \\
CORAL    &90.3 $\pm$ 2.5         &78.0 $\pm$ 2.6         &77.5 $\pm$ 0.4         &X.XX $\pm$ X.XX         &44.7 $\pm$ X.XX         &X.XX $\pm$ X.XX         \\
MMD      &88.0 $\pm$ 1.2         &77.1 $\pm$ 1.2         &76.9 $\pm$ 0.7         &XX.X $\pm$ X.XX         &44.9 $\pm$ X.XX         &X.XX $\pm$ X.XX         \\
\hline
DA-ERM   &91.8 $\pm$ 1.3         &80.1 $\pm$ 0.9         &\textbf{80.5 $\pm$ 0.6}&55.8 $\pm$ X.XX         &\textbf{47.0 $\pm$ X.XX}&\textbf{49.3 $\pm$ X.XX}\\
DA-MMD   &91.6 $\pm$ 1.5         &79.6 $\pm$ 1.4         &79.7 $\pm$ 0.5         &X.XX $\pm$ X.XX         &X.XX $\pm$ X.XX         &X.XX $\pm$ X.XX         \\
DA-CORAL &\textbf{92.0 $\pm$ 1.8}&\textbf{80.2 $\pm$ 1.3}&79.9 $\pm$ 0.8         &X.XX $\pm$ X.XX         &X.XX $\pm$ X.XX         &X.XX $\pm$ X.XX         \\
\hline
\hline
\end{tabular}
\caption{Comparative evaluations on the large-scale benchmark suite.}
\label{tab:exp_large_scale}
\end{table*}
\subsection{Large-Scale Benchmarks}
Our primary evaluation paradigm is the large-scale (real-world) setting, which has been left unexplored in computer vision. Since there are no standardized datasets in the real-world setting, we construct two environments by sub-sampling from existing large-scale vision datasets.
\subsubsection{DG-ImageNet}
The ImageNet~\cite{deng2009imagenet} dataset contains a total of approximately 14M images spread over 22K categories. We subsample 500 categories from the first 5K categories as the \textit{base set}, from which we partition samples from each class into distinct train, val and test subsets. We randomly sample a domain by selecting $K$ (variable) classes randomly from the base set, and then randomly sampling $A$ (variable) points from each class to form the training set for that domain (and correspondingly for the validation and test sets). We sample a total of $N_{\text{tr}}$ training domains. The selection of $A$ points can be done either uniformly (i.e., sample the same number of points $A$ from each class), or with a step function(i.e., some $x\%$ of the classes have large number of samples (\textit{head classes}) and the remainder have small number of classes (\textit{tail classes})) to mimic real-world long-tailed phenomena. Consequently, our overall training set has a non-uniform representation of classes in each domain, along with variation in long-tailed effects.

To construct the test set of domains, we sample $N_{\text{te}} = 10$ domains with $K$ classes only from the set of all classes present in the training set (since we are not tackling zero-shot domain generalization), to ensure that the training data has at least 1 sample from each class (across all training domains)\footnote{We understand that this introduces heterogeneity between the training and test domain distributions, however, since this problem setting does not explicitly create a model for class-wise interactions (as done in zero-shot learning), the alternative baseline would be to reject unseen classes from the test set. Our setting is a more challenging task compared to this alternative, since we introduce more classes in the decision problem.}. Models are run on the combined training set, and hyperparameters are selected based on cross-validation over a separate validation set of domains sampled following the same procedure as the test set (i.e., sampling classes only from the pool of classes selected in the training set).

We report comparisons on this domain in Table~\ref{tab:exp_large_scale}, where $N_{\text{tr}} = 50$ and compare them with the top 3 best-performing benchmarks from the small-scale experiments, as each large-scale experiment takes substantially longer to run and select hyperparameter values accordingly. We additionally remark that we were unable to replicate several algorithms at scale, such as DANN~\cite{ganin2016domain}, Conditional-DANN~\cite{long2018conditional} and MMLD~\cite{pei2018multi}. We see a distinct improvement of \textbf{2.24\%} over ERM, which performs similarly to other benchmarks. 

\subsubsection{Geo-YFCC}
While the synthetic ImageNet dataset does introduce some of the challenges that are commonly encountered in real-world deployment, they are synthetic datasets and cannot be taken as exact substitutes for real-world environments. To this end, we prepared a geographically partitioned benchmark from the YFCC~\cite{thomee2016yfcc100m} dataset. The YFCC100M dataset has approximately 100M images sourced from the photography website Flickr~\cite{flickr_2020} that are annotated with category and geolocation tags. From this data, we filtered images with geotags, and partitioned them by the country of origin (i.e., each \textit{domain} corresponds to data from a country). This provided us with a dataset of 1,261 image classes spread in 61 countries. We use data from (randomly selected) 40 countries as training domains, 7 as validation domains and the remaining 15 as test domains (each domain itself is partitioned into train and test subsets as well). We plan on releasing the complete partitions and annotations in a deanonymized manner upon publication.

This new dataset naturally provides us with several characteristics prevalent in real-world domain generalization (see Appendix for more details). Note that here as well, we were unable to stably replicate many algorithms based on generative modeling as in the ImageNet case, and we selected the top benchmark techniques for a fair evaluation. The results are summarized in Table~\ref{tab:exp_large_scale}. It must be noted that in contrast to ILSVRC12 classification, this problem is substantially more challenging, since we have 1,261 classes with a substantial class imbalance in the training, validation and test sets. Here, we observe that \textit{domain-aware} training provides an average absolute improvement of over \textbf{1\%} (and relative improvement of \textbf{X\%}) in comparison to benchmark techniques. We were unable to obtain statistically significant improvements in other benchmark techniques that operate by domain invariant learning.
\subsection{Ablations}

Studying the behavior of algorithms in the large-scale setting is an interesting and necessary endeavour that has largely been elusive in recent computer vision. We conduct several ablation experiments to examine the behavior of algorithms under various environments.
\subsubsection{Dataset Ablations}
We first examine algorithms as parameters of the dataset are changed. All these ablations are performed on the ImageNet synthetic benchmark with only algorithms that we were easily able to replicate in the large-scale setting.

\textbf{1. Effect of diversity in training data}. We first investigate the effect of more training data on the behavior of algorithms. We first vary the number of available training domains, while sampling the same number of points from each domain\footnote{This experiment involves resampling the test and validation sets for each set of training domains, and therefore the results are only comparable in expectation.}. Next, we repeat the same experiment, however, we subsample points from each domain such that the overall number of training points are the same. The results for these experiments are summarized in Figures~\ref{fig:exp_abl_n_domains} and~\ref{fig:exp_abl_n_domains_fixed}. We observe that all algorithms benefit from additional data, however, the improvements in domain-aware training are larger, which we attribute to diversity in prototype training.

\begin{table}[th!]
\rowcolors{3}{blue!10}{white}
\centering
\footnotesize
\begin{tabular}{ccccc}
\hline
\hline\multirow{2}{*}{Algorithm} & \multicolumn{4}{c}{Accuracy on Test Domains (ImageNet)} \\
      &$N_\trn = 10$&$N_\trn = 20$&$N_\trn = 50$&$N_\trn = 100$ \\
\hline
ERM   & 73.5        & 74.7        & 77.2        & 80.8          \\
Mixup & 73.1        & 75.0        & 77.9        & 80.9          \\
CORAL & 73.0        & 75.2        & 78.0        & 80.2          \\
MMD   & 73.2        & 74.9        & 77.1        & 79.4          \\
\hline
DA-ERM& 74.3        & 75.8        & 80.1        & 83.3          \\ 
\hline
\hline
\end{tabular}
\caption{Effect of number of training domains.}
\label{tab:exp_abl_n_domains}
\end{table}
2. Varying the number of domains while keeping total number of points constant.

\begin{table}[th!]
\rowcolors{3}{blue!10}{white}
\centering
\footnotesize
\begin{tabular}{ccccc}
\hline
\hline\multirow{2}{*}{Algorithm} & \multicolumn{4}{c}{Accuracy on Test Domains (ImageNet)} \\
      &$N_\trn = 10$&$N_\trn = 20$&$N_\trn = 50$&$N_\trn = 100$ \\
\hline
ERM   & 73.5        & 74.4        & 75.0        & 75.1          \\
Mixup & 73.1        & 74.8        & 75.2        & 75.2          \\
CORAL & 73.0        & 75.0        & 75.3        & 75.5          \\
MMD   & 73.2        & 74.2        & 74.5        & 74.8          \\
\hline
DA-ERM& 74.3        & 74.9        & 76.8        & 77.6          \\ 
\hline
\hline
\end{tabular}
\caption{Effect of number of domains, adjusted such that total training data remains constant.}
\label{tab:exp_abl_n_domains_renormalized}
\end{table}
3. Varying the imbalance between classes.

\begin{table}[th!]
\rowcolors{3}{blue!10}{white}
\centering
\footnotesize
\begin{tabular}{cccccc}
\hline
\hline\multirow{2}{*}{Algorithm} & \multicolumn{5}{c}{Accuracy on Test Domains (ImageNet)} \\
      &$x=0\%$&$x=2\%$&$x=5\%$&$x=10\%$&$x=20\%$\\
\hline
ERM   & 48.4  & 49.1  & 51.3  & 54.7   & 60.9   \\
Mixup & 49.5  & 50.8  & 52.5  & 54.9   & 61.4   \\
CORAL & 51.6  & 52.2  & 53.8  & 57.4   & 61.6   \\
MMD   & 50.5  & 52.9  & 55.7  & 58.2   & 61.3   \\
\hline
DA-ERM& 51.1  & 53.8  & 56.2  & 58.8   & 62.2   \\ 
\hline
\hline
\end{tabular}
\caption{Effect of imabalance factor $x$, where $x = 0\%$ implies no points are sampled from tail classes.}
\label{tab:exp_abl_x}
\end{table}
\subsubsection{Algorithm Ablations}

\begin{enumerate}
    \item Effect of prototype dimension.
    \item Effect of prototype training algorithm (feature average, prototype, discriminatory).
\begin{table}[th!]
    \rowcolors{3}{blue!10}{white}
    \centering
    \footnotesize
    \begin{tabular}{cccccc}
    \hline
    \hline\multirow{2}{*}{Dataset} & \multicolumn{5}{c}{Accuracy on Validation Set} \\
                  & Random   & Mean Feature   & Softmax   & Prototypical \\
    \hline
    DG - ImageNet & 80.1     & 80.2           & 80.2      & --   &       \\
    Geo - YFCC    & 49.1     & 49.3           & 49.3      & 49.1  \\
    \hline
    \hline
    \end{tabular}
    \caption{Prototype learning algorithm.}
    \label{tab:exp_abl_proto_training_type}
\end{table}
    \item Effect of prototype set size (i.e., number of points taken to make prototype).
    
\begin{table}[th!]
    \rowcolors{3}{blue!10}{white}
    \centering
    \footnotesize
    \begin{tabular}{cccccc}
    \hline
    \hline\multirow{2}{*}{Dataset} & \multicolumn{5}{c}{Accuracy on Validation Set} \\
                  & 100   & 250   & 500   & 1000   & 2000 \\
    \hline
    DG - ImageNet & 80.1  & 80.2  & 80.2  & --   & --   \\
    Geo - YFCC    & 49.1  & 49.3  & 49.3  & 49.1   & 49.2   \\
    \hline
    \hline
    \end{tabular}
    \caption{Number of points used to construct prototype.}
    \label{tab:exp_abl_num_proto_points}
\end{table}

    \item Effect of bottleneck dimension.
\end{enumerate}

==> sec_intro.tex <==
Real-world machine learning is plagued with numerous issues, most notably the mismatch between training and test data distributions. A model trained on data collected during development may not generalize to deployment settings owing to drift and non-stationarity in the data generation process, introducing error beyond typical finite-sample generalization. More recently, however, machine learning systems are increasingly becoming \textit{decentralized}, i.e., data is held by individual entities, rather than centralized servers. Consider, for example, the medical imaging setting, where a group of hospitals may be collaborating to create a machine learning model. Each data source potentially introduces heterogenous noise by the use of different data collection practices, and this heterogeneity is sustained even during deployment settings (e.g., performing inference on data from different hospitals).

The specific problem of learning and inference on such a heterogenous collection of distinct datasets has been discussed in recent machine learning as the problem of \textit{domain generalization}. The problem setting assumes that the learner is provided with data from several \textit{training domains} and must learn to generalize to unseen distributions~\cite{blanchard2011generalizing}. Recent inquiries into the problem have proposed several different mathematical formalizations as viable models~\cite{gulrajani2020search, ben2010theory}, the most popular of which is \textit{domain-invariant} learning~\cite{baktashmotlagh2013unsupervised, ganin2016domain}. This model assumes that the test data distributions are corrupted variants of the training data distrirbutions, and therefore learning a feature representation that minimizes differences between domains leads to better generalization performance~\cite{li2018deep, li2018deep, muandet2013domain, li2018domain, ghifary2015domain}.

While this approach can be demonstrated to minimize the \textit{average risk} across all domains~\cite{muandet2013domain}, minimizing the \textit{average} risk is not a feasible objective in practice. The problem of domain generalization manifests in real-world applications such as \textit{personalized inference}~\cite{kouw2018introduction} and the earlier example of \textit{federated learning}~\cite{mohri2019agnostic, deng2020adaptive}, where learning a classifer that minimizes the \textit{average risk} across all domains can potentially incur very large risk on any specific domain. Furthermore, recent research has suggested that with high-capacity models, naive fine-tuning (ERM) itself provides better or comparable performance on a wide variety of domain generalization problems than any \textit{domain-invariant} algorithm~\cite{gulrajani2020search}, casting doubt on \textit{domain-invariant} strategies for large-scale or personalized inference.

Motivated by this reasoning, we examine the domain generalization problem in the context of such real-world and large-scale tasks. We consider an alternate \textit{domain-aware} classification approach, that utilizes unsupervised signals to characterize each domain itself, inspired by the extensive literature on \textit{kernel mean embeddings} for probability distributions. Our contributions can be summarized as follows.

1. In contrast to existing domain-invariant approaches, we develop a framework for \textit{domain-aware} classification for domain generalization. We leverage the theory of risk minimization with kernel mean embeddings of distributions~\cite{gretton2012kernel} and provide a rigorous theoretical framework for \textit{domain-aware} domain generalization, supplementing the literature on invariant approaches~\cite{ben2010theory}.

2. Building on this framework, we propose an algorithm for training \textit{domain-aware} neural network classifiers. Our algorithm repurposes low-shot \textit{prototypical network learning}~\cite{snell2017prototypical, fort2017gaussian} to create domain embeddings which are then provided as supplementary input to pre-trained neural network classifiers. We provide a rigorous theoretical motivation to the design choices for our algorithm as well.

3. We introduce the first set of \textit{real-world} domain generalization benchmarks, dubbed \textbf{Geo-YFCC}, which contains 40 training, 7 validation and 15 test domains, with an overall $XXXXX$ samples. This dataset is constructed from the popular benchmark YFCC100M~\cite{thomee2016yfcc100m}, partitioned based on geographical tags. This dataset exhibits several characteristics of \textit{domain shift}~\cite{li2017deeper} and \textit{label shift}~\cite{azizzadenesheli2019regularized}, including long-tailed label distributions common in real-world classification problems~\cite{zhang2017range, xiang2020learning, cao2020domain}. Our proposed benchmark is substantially more challenging than the small-scale benchmarks incumbent in computer vision research.

4. On small-scale benchmarks and more notably, 2 large-scale benchmarks, we demonstrate the strength of naive ERM and \textit{domain-aware} classification over other \textit{domain-invariant} approaches. In addition to the viability of \textit{domain-aware} classification, this suggests, in corroboration with the claims of Gulrajani and Lopez-Paz~\cite{gulrajani2020search}, that stronger model selection practices and larger benchmarks can shed more light on the problem of domain generalization.

Our paper is organized as follows. We first present a summary of the relevant related research to our contributions, and then provide a brief (informal) intuition behind \textit{domain-aware} classification. We then formally introduce the formal framework, associated error bounds, and the primary algorithm. We then present an overview of the experimental setup, small-scale datasets, and the YFCC100M and ImageNet-based benchmarks and our experimental results on these benchmarks. Finally, we provide concluding remarks and a discussion on the future directions of research.


==> sec_intro_dhruv.tex <==
\begin{figure}[t!]
\centering
\includegraphics[width=0.75\linewidth]{intuition.pdf}
\caption{A visual representation of the intuition behind our algorithm on a training set with 8 domains. Typically, for any test domain $D_T$, the \textit{universal} classifier $\hat f_*$ may be far from the \textit{feasible set}, which can have low error on $D_T$.}\label{fig:intuition}
\end{figure}

Real-world machine learning is plagued with numerous issues, most notably the mismatch between training and deployment data distributions, often due to drift and non-stationarity in the data generation process. Machine learning systems are also increasingly becoming \textit{personalized}, i.e., predictions are held by individual entities (geographies, users, etc.), rather than centralized servers due to privacy constraints. 
% Consider, for example, the medical imaging setting, where a group of hospitals may be collaborating to train a model. Each data source potentially introduces heterogeneous noise by the use of different data collection practices, and this heterogeneity is sustained even during deployment settings (e.g., performing inference on data from different hospitals).
The specific problem of learning and inference on such a heterogeneous collection of distinct datasets has been discussed in machine learning literature as the problem of \textit{domain generalization}. The problem setting assumes that the learner is provided with data from several \textit{training} distributions (domains) and must learn to generalize to unseen \textit{test} domains~\cite{blanchard2011generalizing}. Recent inquiries into the problem have proposed several different mathematical formalizations as viable approaches~\cite{gulrajani2020search, ben2010theory}, the most popular of which is \textit{domain-invariant} learning~\cite{baktashmotlagh2013unsupervised, ganin2016domain}. This approach extends the formalism of the related problem of \textit{domain adaptation}, where a model trained in a \textit{source} domain must be adapted to run in a \textit{target} domain. Invariant methods propose learning feature representations that are invariant to the underlying domains, and hence create classifiers that generalize to unseen test distributions~\cite{li2018deep, li2018deep, muandet2013domain, li2018domain, ghifary2015domain}. 

While \textit{domain-invariant} approaches can be used to learn a \textit{universal} classifier to minimize the \textit{average risk} across all domains~\cite{muandet2013domain}, minimizing the \textit{average} risk may not a feasible objective in practice. Consider Figure~\ref{fig:intuition} for example. For many real-world domain generalization applications such as \textit{personalized inference}~\cite{kouw2018introduction} and  \textit{federated learning}~\cite{mohri2019agnostic, deng2020adaptive}, the set of domains can be quite diverse. Hence, learning a classifier that minimizes the \textit{average risk} across all domains can potentially incur very large risk (referred as {\it{"non-adaptive gap"}} in Figure~\ref{fig:intuition}) on any specific domain. Furthermore, recent research~\cite{} has suggested that with high-capacity models, naive fine-tuning (ERM) done by combining data from all the seen training domains itself provides better or comparable performance on a wide variety of domain generalization problems than any \textit{domain-invariant} algorithm~\cite{gulrajani2020search}.

% The problem of domain generalization manifests in real-world applications such as \textit{personalized inference}~\cite{kouw2018introduction} and the earlier example of \textit{federated learning}~\cite{mohri2019agnostic, deng2020adaptive}, where learning a classifier that minimizes the \textit{average risk} across all domains can potentially incur very large risk on any specific domain. Furthermore, recent research has suggested that with high-capacity models, naive fine-tuning (ERM) itself provides better or comparable performance on a wide variety of domain generalization problems than any \textit{domain-invariant} algorithm~\cite{gulrajani2020search}, casting doubt on the \textit{domain-invariant} strategies for large-scale or personalized inference.

In this work, we examine the domain generalization problem in the context of such real-world and large-scale tasks and consider an alternate \textit{domain-aware} classification approach. For an unseen domain, neighboring domains with similar data distributions (referred as {\textit{"feasible set"}} in Figure~\ref{fig:intuition}) should be better candidates to build a representative model. Motivated by this reasoning, we propose a two step approach: a) Build a manifold of domains whose each point is a domain and distance between the two points (domains) represent the similarity of their data distributions, and, b) Use the domain's manifold representation as supplementary signal to the neural-net model so that it can generalize to unseen domains. We assume that at inference time, we have small amount of unsupervised data from an unseen domain and use it to build its manifold representation.

Our contributions can be summarized as follows.

1. In contrast to existing domain-invariant approaches, we develop a framework for \textit{domain-aware} classification for domain generalization. We leverage the theory of risk minimization with kernel mean embeddings of distributions~\cite{gretton2012kernel} and provide a rigorous theoretical framework for \textit{domain-aware} domain generalization, supplementing the literature on invariant approaches~\cite{ben2010theory}.

2. Building on this framework, we propose an algorithm for training \textit{domain-aware} neural network classifiers. Our algorithm repurposes low-shot \textit{prototypical network learning}~\cite{snell2017prototypical, fort2017gaussian} to create domain embeddings which are then provided as supplementary input to pre-trained neural network classifiers. We provide a rigorous theoretical motivation to the design choices for our algorithm as well.

3. We introduce the first set of \textit{real-world} domain generalization benchmarks, dubbed \textbf{Geo-YFCC}, which contains 40 training, 7 validation and 15 test domains, with an overall $XXXXX$ samples. This dataset is constructed from the popular benchmark YFCC100M~\cite{thomee2016yfcc100m}, partitioned based on geographical tags. This dataset exhibits several characteristics of \textit{domain shift}~\cite{li2017deeper} and \textit{label shift}~\cite{azizzadenesheli2019regularized}, including long-tailed label distributions common in real-world classification problems~\cite{zhang2017range, xiang2020learning, cao2020domain}. Our proposed benchmark is substantially more challenging than the small-scale benchmarks incumbent in computer vision research.

4. On small-scale benchmarks and more notably, 2 large-scale benchmarks, we demonstrate the strength of naive fine-tuning (ERM) and \textit{domain-aware} classification over other \textit{domain-invariant} approaches. In addition to the viability of \textit{domain-aware} classification, this suggests, in corroboration with the claims of Gulrajani and Lopez-Paz~\cite{gulrajani2020search}, that stronger model selection practices and larger benchmarks can shed more light on the problem of domain generalization.

Our paper is organized as follows. We first present a summary of the relevant related research to our contributions, and then provide a brief (informal) intuition behind \textit{domain-aware} classification. We then formally introduce the formal framework, associated error bounds, and the primary algorithm. We then present an overview of the experimental setup, small-scale datasets, and the YFCC100M and ImageNet-based benchmarks and our experimental results on these benchmarks. Finally, we provide concluding remarks and a discussion on the future directions of research.


==> sec_intro_v2.tex <==
\begin{figure}[t!]
\centering
\includegraphics[width=0.75\linewidth]{intuition.pdf}
\caption{A visual heuristic for \textit{adaptive} domain generalization. Here we denote by $\hat f_i$ the optimal ERM classifier in a class $\cF$ for domain $i$ (out of $8$ total domains). Typically, for any new test domain $D_T$, the optimal \textit{universal} classifier $\hat f_*$ may be far from the \textit{feasible set}, which can have low error on $D_T$.}\label{fig:intuition}
\end{figure}

% Real-world machine learning is plagued with numerous issues, most notable being the mismatch between training and deployment data distributions, often due to drift and non-stationarity in the data generation process. In many settings, such systems are also increasingly becoming \textit{personalized}, i.e., predictions are being customized to individual entities (geographies, users, etc.), rather than universal, centralized inference.
% Consider, for example, the medical imaging setting, where a group of hospitals may be collaborating to train a model. Each data source potentially introduces heterogenous noise by the use of different data collection practices, and this heterogeneity is sustained even during deployment settings (e.g., performing inference on data from different hospitals).
The problem of learning from a heterogenous collection of distinct sources (or domains) has been discussed extensively in machine learning literature as the problem of \textit{domain generalization}. The problem setting assumes that the learner is provided with data from several \textit{training} domains and must learn to generalize to unseen \textit{test} domains~\cite{blanchard2011generalizing}. Recent inquiries into this problem have proposed various mathematical formalizations for the problem~\cite{gulrajani2020search, ben2010theory}, the most popular of which is \textit{domain-invariant} learning~\cite{baktashmotlagh2013unsupervised, ganin2016domain}. This approach extends formalism from the related problem of \textit{domain adaptation}, where a model trained in a \textit{source} domain must be adapted to run in a \textit{target} domain. Invariant methods propose learning feature representations that are invariant to the underlying domains, and hence create a \textit{universal} classifier that generalize to unseen test distributions~\cite{li2018deep, li2018deep, muandet2013domain, li2018domain, ghifary2015domain}. 

A rich literature demonstrates that domain-invariant \textit{universal} classifiers typically minimize the \textit{average risk} across all domains~\cite{muandet2013domain}. However, a universal classifier that minimizes the \textit{average} risk may not a feasible objective in practice, as demonstrated heuristically in Figure~\ref{fig:intuition}. The optimal classifiers for any \textit{specific} test domain can lie far from the \textit{universal} classifier, as seen in the figure (i.e., the \textit{adaptivity gap}). For any domain, we would like to \textit{adapt} the classifier such that it is close to the optimal function for the test domain (i.e., within the \textit{feasible set}).
% For many real-world domain generalization applications such as \textit{personalized inference}~\cite{kouw2018introduction} and  \textit{federated learning}~\cite{mohri2019agnostic, deng2020adaptive}, the set of domains can be quite diverse. Hence, learning a classifer that minimizes the \textit{average risk} across all domains can potentially incur very large risk (referred as {\it{"non-adaptive gap"}} in Figure~\ref{fig:intuition}) on any specific domain. 

% Furthermore, recent research~\cite{} has suggested that with high-capacity models, naive fine-tuning (ERM) done by combining data from all the seen training domains itself provides better or comparable performance on a wide variety of domain generalization problems than any \textit{domain-invariant} algorithm~\cite{gulrajani2020search}.

% The problem of domain generalization manifests in real-world applications such as \textit{personalized inference}~\cite{kouw2018introduction} and the earlier example of \textit{federated learning}~\cite{mohri2019agnostic, deng2020adaptive}, where learning a classifer that minimizes the \textit{average risk} across all domains can potentially incur very large risk on any specific domain. Furthermore, recent research has suggested that with high-capacity models, naive fine-tuning (ERM) itself provides better or comparable performance on a wide variety of domain generalization problems than any \textit{domain-invariant} algorithm~\cite{gulrajani2020search}, casting doubt on the \textit{domain-invariant} strategies for large-scale or personalized inference.

In this paper, we examine the domain generalization problem in the context of such real-world and large-scale tasks and consider the aforementioned \textit{domain-adaptive} classification approach. To create a generalizable adaptive classifier, however, it is necessary that some information about the test domain (via unsupervised samples) be present \textit{at test time}. This assumption is trivial, as there are by definition unsupervised samples in the test set, which we leverage to \textit{adapt} a general classifier to that domain. Our approach is two-fold: first, we use a \textit{low-shot} unsupervised algorithm to embed domains into a vector space using only a very small number of samples, and then leverage these \textit{domain embeddings} as supplementary signals to learn a \textit{domain-adaptive} classifier such that it generalizes to unseen domains. Our contributions can be summarized as follows.

1. We propose an algorithm for training \textit{domain-adaptive} neural networks. Our algorithm repurposes low-shot \textit{prototypical learning}~\cite{snell2017prototypical, fort2017gaussian} to create \textit{domain embeddings} which are then provided as supplementary inputs to pre-trained neural network classifiers. Our algorithm is built on rigorous design choices derived from novel theoretical results for the kernel mean embeddings of distributions.

2. We develop an algorithmic framework for \textit{adaptive} classification for domain generalization. Our framework leverages the theory of risk minimization with kernel mean embeddings of distributions~\cite{gretton2012kernel}, supplementing the vast literature on invariant approaches~\cite{ben2010theory, arjovsky2019invariant, albuquerque2019generalizing}.

3. We introduce the first large-scale, real-world domain generalization benchmark, dubbed \textbf{Geo-YFCC}, which contains 40 training, 7 validation and 15 test domains, with an overall $XXXXX$ samples. This dataset is constructed from the popular YFCC100M~\cite{thomee2016yfcc100m} dataset, partitioned by geographical tags. It exhibits several characteristics of \textit{domain shift}~\cite{li2017deeper}, \textit{label shift}~\cite{azizzadenesheli2019regularized}, and long-tailed class distributions common in real-world classification~\cite{zhang2017range, xiang2020learning, cao2020domain}. This benchmark is substantially more challenging than the small-scale benchmarks incumbent in computer vision.

4. On existing benchmarks and notably, 2 large-scale benchmarks, we demonstrate the strength of fine-tuning (ERM) with \textit{domain-adaptive} classification over other \textit{domain-invariant} approaches.
In addition to the effectiveness of adaptive classification, this suggests, along with the claims of Gulrajani and Lopez-Paz~\cite{gulrajani2020search} that rigorous model selection and large benchmarks are essential in understanding domain generalization, where naive ERM can be a powerful baseline in a suitable function class.

% Our paper is organized as follows. We first present a summary of the relevant related research to our contributions, and then provide a brief (informal) intuition behind \textit{domain-aware} classification. We then formally introduce the formal framework, associated error bounds, and the primary algorithm. We then present an overview of the experimental setup, small-scale datasets, and the YFCC100M and ImageNet-based benchmarks and our experimental results on these benchmarks. Finally, we provide concluding remarks and a discussion on the future directions of research.


==> sec_method.tex <==
\begin{figure*}[htb]
\centering
\includegraphics[width=\linewidth]{main.pdf}
\caption{A visual representation of our two-step training pipeline. Figure A describes the prototypical training process (Step 1), which is followed by training the \textit{adaptive} classifier (Figure B).}
\label{fig:myfigure}
\end{figure*}
Our approach can be coarsely summarized in two steps. First, we learn a neural network $\Phi_\cD :\cX \rightarrow \bbR^{d_D}$, parameterized by weights $\btheta$, and then compute the kernel mean embedding (KME) $\mu$ of each training domain $\widehat D \in \cS_\trn$ as:
\begin{equation}
    \mu(\widehat D) = \frac{1}{n}\sum_{\x \in \widehat D} \Phi_\cD(\x ; \btheta).
\end{equation}
Once we have the KMEs for each training domain, we then create the \textit{augmented training set} by concatenating the corresponding KME for each input image. Finally, we have the training set $\widetilde\cS_\trn = \cup_{i=1}^{N} \widetilde D^i_\trn$, where, 
\begin{equation}
\widetilde D^i_\trn = \left(\x_{ij}, \mu(\widehat D_\trn^i), y_{ij}\right)_{j=1}^{n}.
\label{eqn:augmented_dataset}
\end{equation}

The second step is to then train the \textit{domain-adaptive} classifier $F$, i.e., a neural network with weights $\bomega$ that takes the augmented input $(\x, \mu(D))$ for any input-domain combination and predicts the class label $y$. In the next section (Section~\ref{sec:prototype}) we describe the design principles behind learning $\Phi_\cD$, followed by those of $F$ (Section~\ref{sec:training_inference}).

% In our approach, we directly train a \textit{domain-aware} neural network $g: \bbR^d \times \bbR^{d_D} \rightarrow [K]$. For any input image $\x$ from domain $\cD$, $g$ takes in the \textit{augmented} input $(\x, \phi(\cD; \btheta^*))$, which is composed of the input $\x$ and the corresponding domain prototype $\phi(\cD; \btheta^*)$ obtained from the previous section, and predicts the class label $\hat y$ as output. The neural network architecture is described in Figure~\ref{fig:net_architecture}.

% $g$ is a composition of an image feature extractor ($\Phi_X$) whose output is concatenated with the domain prototype $\Phi(\cD)$ and fed into a series of non-linear layers ($\fK$) to produce the final output. The domain-aware neural network parameters are denoted by $\bomega$. The complete function $f$ therefore is parameterized by both $\bomega$ and $\btheta$ and is described as $f(\x, \cD; \bomega, \btheta) = g(\x, \phi(\cD; \btheta); \bomega)$.
\subsection{Domain Prototypes}
\label{sec:prototype}
To be useful in classification, we require that the KME $\mu$ satisfy two central criteria:\\
\textit{\textbf{A. Expressivity}}: $\mu$, and consequently, $\Phi_\cD$, must be expressive, i.e., for two domains $D$ and $D'$, $\lVert \mu(D) - \mu(D') \rVert_2$ must be large if they are very distinct (i.e., domain shift), and small if they are similar. For example, if $\Phi_\cD$ is constant, the KME will provide no additional information about $D$, and we can expect the \textit{expected risk} $L(F)$ itself to be large in this case, equivalent to non-adaptive classification.\\
\textit{\textbf{B. Consistency}}: The domain feature $\phi$ must have little dependence on both the choice, and the number of empirical samples $\x$ used to construct it. This is desirable as during both training and testing, we only have access to the empirical distribution $\widehat{D}$ corresponding to any domain $D$. This claim is made more rigorous by the following result that characterizes the deviation $\lVert f(\cdot, \mu(\widehat{D})) - f(\cdot, \mu(D)) \rVert_\infty$.
\begin{theorem}[Approximation of KME]
Consider domain $D$, and let $\widehat{D}$ be the distribution of $n$ samples from $\cX$ drawn according to $D$. Assume bounds $\lVert\Phi_\cD(\x)\rVert_2 \leq B$ and $\bbE_{\x \sim D}[\lVert \Phi_\cD(\x) \rVert_2^2] \leq \sigma^2$. Then, we have for any $f \in \cB_\kappa(R)$ (ref. Theorem~\ref{thm:risk_bound}) with probability at least $1-\delta$,
\begin{equation*}
    \Delta_f(\mu(D), \mu(\widehat D)) \leq \mathcal O\left(\frac{R\log(\frac{1}{\delta})}{n} + \frac{R\sigma}{B} \sqrt{\frac{\log(\frac{1}{\delta})}{n}}\right).
\end{equation*}
\label{thm:feature_variance}
Where $\Delta_f(\mu(D), \mu(\widehat D)) = \lVert f(\cdot, \mu(\widehat{D})) - f(\cdot, \mu(D)) \rVert_\infty$.
\end{theorem}
Theorem~\ref{thm:feature_variance} suggests that for an ideal $\mu$, the feature $\Phi_\cD$ must have small variance $\sigma^2$ over any domain $D$ so that $\mu(\widehat{D})$ is close to $\mu(D)$ for small $n$. In the case when $\cD$ is finite, an obvious choice for $\Phi_\cD$ can be the vertices of an $|\cD|$-dimensional simplex. For any arbitrary $\cD$, however, we cannot make \textit{a priori} assumptions about $\Phi_\cD$, and it is reasonable to learn $\Phi_\cD$ from the data samples themselves.

The central idea therefore is that we want to learn $\Phi_\cD$ such that for any sample $\x$ from domain $D$, $\Phi_\cD(\x)$ is strongly clustered around the KME $\mu(D)$, and that the KMEs for different domains are positioned adequately apart. These exact constraints have been explored previously in the area of low-shot classification, by an algorithm known as \textit{prototypical learning}~\cite{snell2017prototypical}. Prototypical learning learns a set of \textit{prototypes} (ref. KMEs) for each class in a low-shot classification problem, and predicts the label of a new point as the class label of its nearest prototype.

The resultant space spanned by the embedding function $\Phi_\cD$ induces a clustering of the input space $\cX$ in terms of the Bregman divergence in the exponential family of the model parameters (in our case, $\btheta$, see Section 2.3 of Snell~\etal\cite{snell2017prototypical}), and it is this form of partitioning of the input space based on clusters corresponding to domains that would encode information about $\cD$. We therefore adopt a \textit{domain-level} prototypical learning model, where we essentially run the prototypical network algorithm (Algorithm 1 of~\cite{snell2017prototypical}) but using the domains identities as the output labels.

We provide the complete prototypical training pipeline in the Appendix for brevity and only discuss the keys steps of the algorithm here. Prototypical training proceeds by randomly sampling a batch of points from each domain, and running a feedforward operation of $\Phi_\cD$ on them. Then, a random subset of points from each domain are used to create an approximation of $\mu(\widehat D)$ for each domain $D$, and the remaining points are used for $N$-way classification. Prototypical networks produce a distribution over the domains for any input point $\x$ based on a softmax of distances to the prototypes for each training domain:
\begin{align}
    p_\btheta(\x \in D) = \frac{\exp\left(-\lVert \mu(\widehat D) - \Phi_\cD(\x)\rVert_2^2 \right)}{\sum_{i=1}^{N} \exp\left(-\lVert \mu(\widehat D_\trn^i) - \Phi_\cD(\x)\rVert_2^2\right)}.
\end{align}
Learning proceeds by minimizing the negative log-probability $J(\btheta) = -\log p_\btheta(\x \in D)$ for the correct domain via SGD. Once this training is complete, we obtain the final neural network parameters $\btheta^*$. For each domain $\widehat D_\trn^i$, the \textit{domain prototype} can then be constructed as:
\begin{equation}
    \mu(\widehat D_\trn^i) := \frac{1}{n}\sum_{j=1}^{n} \Phi_\cD(\x; \btheta^*).
    \label{eqn:final_prototype}
\end{equation}
We repeat \textit{only} Equation~\ref{eqn:final_prototype} for each of the test domains as well. It is important to note that this is not the \textit{transductive learning} setting, where access to the test domains is provided \textit{a priori}. Therefore, we \textbf{do not} include the test domains in the prototypical training process.
\subsection{Training and Inference}
\label{sec:training_inference}

\textbf{Training}. Our training process has two steps. We first train the domain prototypical network parameters $\btheta$ using the inputs $\x$ from each domain. Since we do not utilize any class labels, the prototypical training process is entirely unsupervised (as long as we are provided the inputs partitioned by their source domains). Additionally, our method does not require that the unsupervised samples used to train the domain prototypical classifier be the same as the training set for the \textit{domain-adaptive} model.  

Once the parameters $\btheta^*$ have been obtained, we compute the domain prototypes for each of the $N$ training domains present (according to Equation~\ref{eqn:final_prototype}). We then create the \textit{augmented training set} $\widetilde \cS_\trn$ by concatenating the corresponding domain prototype for each input image (Equation~\ref{eqn:augmented_dataset}). This augmented training set is used to train the \textit{domain-aware classifier} weights $\bomega$. The classifier is trained via a regular cross-entropy loss minimization (ERM).

\textbf{Inference}. During testing, we first compute the domain prototypes for each of the test domains (Equation~\ref{eqn:final_prototype}, we can also use a small sub-sample of the total test set for this), and produce predictions via $F$.

\textbf{Online Inference}. Alternatively, it is possible to decouple the prototype construction and inference procedures in the test phase (since we can use unsupervised samples from a domain obtained \textit{a priori} to construct prototypes). In this setting, we can use a distinct set of $n_p$ points to construct the domain prototype for each test domain. We can see directly from Theorem~\ref{thm:feature_variance} that for any Lipschitz loss function, the maximum disparity between classification using the optimal prototype (i.e., formed with knowledge of $\cD$) and the $n_p$-sample approximation is (with high probability) at most $\widetilde{\cO}\left(n_p^{-\alpha} + (\sigma_P/n_p)^{-\alpha/2}\right)$, which is small when $\sigma_P$ is small, i.e., the prototype is consistent.


==> sec_motivation_background.tex <==
\textbf{Motivation}. We begin by provifing an (informal) intuition for our approach, followed by a more rigorous technical treatment of the method. We assume that each \textit{domain} $D \in \cD$ is a probability distribution over $\cX \times \cY$, i.e., the product of input space $\cX$ and output space $\cY$, and there exists a \textit{mother} distribution $\fP$ which is a probability distribution over the space of domains $\cD$. Therefore, every \textit{training domain} $\widehat D(n)$ is sampled by first sampling a domain $D$ from $\fP$, and then sampling $n$ points ($X$ and $Y$) from $\cX \times \cY$ following $D$. A training set can then be formed by taking the union of $N$ such domains $(\widehat{D}_i(n))_{i=1}^N$. Correspondingly, any test domain $\widehat D_T(n_T)$ is also characterized by first drawing a sample $D_T \sim \cD$ and then drawing $n_T$ samples from $D_T$, discarding the labels.

Now, consider a family of functions $\cF$ such that for each $D \in \cD$, the optimal classifier $f_D$ (for some loss function $\ell$) can be given by $ f_D = \argmin_{f \in \cF} \bbE_{(\x, y) \sim D}[\ell(f(\x), y)]$. When learning the function $\widehat D(n)$ (i.e., from $n$ empirical samples of $D$), we denote the ERM solution as $\hat f_D = \argmin_{f \in \cF} \bbE_{(\x, y) \sim \widehat D(n)}[\ell(f(\x), y)]$. Now, the optimal ERM classifier for each $\widehat{D}_i(n)$ can be given by $\hat f_i$, and the \textit{universal} optimal ERM classifier can be given by $\hat f_*$, i.e., $\hat f_* = \argmin_{f \in \cF} \bbE_{D \sim \fP}\bbE_{\x, y \sim D}[\ell(f(\x), y)]$.

Now, when we are provided with samples from an unseen test domain $D_T$, typically, the optimal classifier for $D_T$ within $\cF$ may be far from the (non-adaptive) universal classifier $\hat f_*$, a distance which we call the ``adaptivity gap''. A visual heuristic representation of the above intuition is provided in Figure~\ref{fig:intuition}. Ideally, we would like the classifier to be chosen from the ``feasible set'' for $D_T$, such that it obtains lower error. Note that as illustrated in the figure, the \textit{adaptivity gap} may be large even when the training set contains samples from the \textit{feasible set} (in the figure, this corresponds to functions $\hat f_7$ and $\hat f_8$), since different domains can have different impacts on the invariant classifier learnt.

Our approach attempts to minimize this discrepancy by learning an \textit{adaptive} classifier, i.e., a function $F: \mathcal X \times \mathcal D \rightarrow \mathcal Y$ that takes \textit{both} the point $\x$ and the domain $D$ of $\x$ as inputs when making predictions. Our goal is to make sure that for any input domain $D_T$, the resulting classifier $F(\cdot, D_T)$ from $F$ lies in the feasible set of $D_T$.

The main challenge in creating such a function $F$ is that it is non-trivial to learn a function on the space of probability distributions themselves. To alleviate this issue, we look to the literature on kernel mean embeddings (KME)~\cite{muandet2016kernel}, a mathematical formalization that allows us to represent a probability distribution as the average feature vector computed on samples drawn from the probability distribution itself. That is, the idea is to laern a function $\Phi$ that maps the empirical domain to a finite vector, i.e., $\Phi : D \rightarrow \bbR^{d_\cD}$. With a suitable domain embedding $\Phi$, we can learn a neural network $F$ directly over the \textit{augmented input} $(\x, \Phi(\widehat D))$, where $\x$ is a point from the domain $\widehat D$, via regular ERM.

\textbf{Preliminaries}. Let $\cX \subset \bbR^d$ be a compact input space, $\mathcal Y \in [-1, 1]$ be the output space, and $\cD$ denote the set of all probability distributions over the measurable space $(\cX \times \cY, \Sigma)$, where $\Sigma$ is the $\sigma$-algebra of subsets of $\cX \times \cY$\footnote{Additionally, we assume there exists sets of probability distributions $\cD_\cX$ and $\cD_{\cY | \cX}$ such that for any sample $D \in \cD$ there exist samples $D_X \in \cD_\cX$ and $D_{Y|X} \in \cD_{\cY|\cX}$ such that $D = D_X \bullet D_{Y|X}$ (this characterization is applicable under suitable assumptions, see Sec. 3 of~\cite{blanchard2011generalizing}).}. We assume that there exists a probability measure $\fP$ over $\cD$ and each \textit{domain} $D$ is an i.i.d. sample from $\cD$, according to $\fP$. The \textit{training set} is generated as follows. Nature samples $N$ domains $D_{\trn}^{1}, ..., D_{\trn}^{N}$ from $\fP_{\cX\times\cY}$ according to $\fP$. For each domain $D_i$, nature further samples $n$ samples of $(\x, y) \sim D_i$ each, giving us the empirical measure $\widehat D_i$ for each domain $D_i$. The \textit{training dataset} can be denoted as $\cS_\trn = \cup_{i=1}^N \widehat D^i_\trn$, which contains a total of $nN$ samples\footnote{We assume that $n$ samples are selected from each of the $N$ training domains for simplicity, however, our analysis holds for unique sample counts.}. Each \textit{test} domain is sampled similarly to the training domain, where nature first samples a probability distribution $D_T \sim \fP$, and then samples $n_T$ points $(\x_j^{T}, y_j^{T})_{j \in [n_T]}$ from $D_T$ to form the empirical measure $\widehat D_T$ (i.e., test domain). 

